Gait Switching and Enhanced Stabilization of Walking Robots with Deep Learning-based Reachability: A Case Study on Two-link Walker

Learning-based approaches have recently shown notable success in legged locomotion. However, these approaches often lack accountability, necessitating empirical tests to determine their effectiveness. In this work, we are interested in designing a learning-based locomotion controller whose stability can be examined and guaranteed. This can be achieved by verifying regions of attraction (RoAs) of legged robots to their stable walking gaits. This is a non-trivial problem for legged robots due to their hybrid dynamics. Although previous work has shown the utility of Hamilton-Jacobi (HJ) reachability to solve this problem, its practicality was limited by its poor scalability. The core contribution of our work is the employment of a deep learning-based HJ reachability solution to the hybrid legged robot dynamics, which overcomes the previous work's limitation. With the learned reachability solution, first, we can estimate a library of RoAs for various gaits. Second, we can design a one-step predictive controller that effectively stabilizes to an individual gait within the verified RoA. Finally, we can devise a strategy that switches gaits, in response to external perturbations, whose feasibility is guided by the RoA analysis. We demonstrate our method in a two-link walker simulation, whose mathematical model is well established. Our method achieves improved stability than previous model-based methods, while ensuring transparency that was not present in the existing learning-based approaches.

==> notes_for_plan.tex <==
\note{Our goal is to}

- provide maximal regions of attraction for theoretical analysis of bipedal robots push recovery

- Deriving optimal controller based on HJ value function to stabilize each gait with minimum time-to-reach.

- To showcase the effectiveness of our approach in comparison to the existing NMPC gait transition method for push recovery???



\note{Several Tasks for Our Paper}

1. show our parameterized BRTs

   * 3d picture

     previous 2d slice and a new dimension for parameter

   * contour plot: our learned target function

   

2. show our controller(predictive controller)

   states within brt:

   * trajectory map: states within brt converge within 3 steps
   * (*) shaking lgV (imply the importance of our predictive controller)
   * (*)mc simulation results: successful rate (opt vs osp)

   states outside of brt:

   * gait perturbation (overlap picture)

   * gait transition(from uncontrollable to controllable)

     how to visualize this in the paper???

   

3. make comparisons:

   * NMPC for gait transition vs. our proposed optimal controller

     use mc results to prove our method is better?(though we need a predefined fixed gait)

\note{\textbf{Outline}}

% possible headline:

% **Deep Learning-Based Reachability Analysis for Gait Switching and Enhanced Stabilization**

1. Introduction

   push recovery literature review

   seldom provide theoretical analysis on the regions of attraction

   how far can we push the robots? when will the robots be able to go back to normal?

2. contribution

   1. verify ROA of each gait, 

   2. optimal controller as stabilizing controller. 

      (optional)more accurate than dynamic programming based HJ

      better successful rate than mpc 

   3. strategy to switch between gaits based on the verified ROAs 

   4. 

      

3. background

   * hybrid system reachability(*) 
   value remapping
   
   * problem setup
   * compass gait and push recovery

4. Regions of Attraction Analysis for Gaits

   Explain how we use parameterized deepreach to calculate BRTs and their meaning
    \begin{enumerate}
        \item 1. what is parameterization
        \item 2. seq2seq training
        \item 3. value remapping loss and other losses
        \item 4. learning the target function (optional picture)
    \end{enumerate}

    
   Explain how they could be used in push recovery

   *contour plot(optional): our learned target function*

   *3d picture of BRTs*(optional): previous 2d slice and a new dimension for parameter

   **overlap picture**

   

5. make disturbed Robots back to control

   For perturbed states still within BRT

   * trajectory map: states within brt converge within 3 steps
   * (optional) shaking lgV (imply the importance of our predictive controller)
   * 

   Perturbed states are outside BRT

   * gait perturbation

     trajectory perturbation

   * gait transition(from uncontrollable to controllable)

    gait switching algorithm
    
     how to visualize this in the paper???

     
   NMPC for gait transition vs. our proposed optimal controller

   * use mc simulation to prove our method is better?(though we need a predefined fixed gait)
